RIS-Assisted Sensing: A Nested Tensor Decomposition-Based Approach

We study a monostatic multiple-input multiple-output sensing scenario assisted by a reconfigurable intelligent surface using tensor signal modeling. We propose a method that exploits the intrinsic multidimensional structure of the received echo signal, allowing us to recast the target sensing problem as a nested tensor-based decomposition problem to jointly estimate the delay, Doppler, and angular information of the target. We derive a two-stage approach based on the alternating least squares algorithm followed by the estimation of the signal parameters via rotational invariance techniques to extract the target parameters. Simulation results show that the proposed tensor-based algorithm yields accurate estimates of the sensing parameters with low complexity.

==> addons/acronym.tex <==
\begin{acronym}
        \acro{RIS}{reconfigurable intelligent surface}
        \acro{irs}{intelligent reflecting surface}
        \acro{PARAFAC}{parallel factor}
        \acro{TALS}{trilinear alternating least squares}
        \acro{BALS}{bilinear alternating least squares}
        \acro{DF}{decode-and-forward}
        \acro{AF}{amplify-and-forward}
        \acro{CE}{channel estimation}
        \acro{RF}{radio-frequency}
        \acro{THz}{Terahertz communication}
        \acro{EVD}{eigenvalue decomposition}
        \acro{CRB}{Cramér-Rao lower bound}
        \acro{CSI}{channel state information}
        \acro{BS}{base station}
        \acro{MIMO}{multiple-input multiple-output}
        \acro{NMSE}{normalized mean squared error}
        \acro{2G}{Second Generation}
        \acro{3G}{3$^\text{rd}$~Generation}
        \acro{3GPP}{3$^\text{rd}$~Generation Partnership Project}
        \acro{4G}{4$^\text{th}$~Generation}
        \acro{5G}{5$^\text{th}$~Generation}
        \acro{6G}{6$^\text{th}$~generation}
        \acro{E-TALS}{\textit{enhanced} TALS}
        \acro{UT}{user terminal}
        \acro{UTs}{users terminal}
        \acro{LS}{least squares}
        \acro{KRF}{Khatri-Rao factorization}
        \acro{KF}{Kronecker factorization}
        \acro{MU-MIMO}{multi-user multiple-input multiple-output}
        \acro{MU-MISO}{multi-user multiple-input single-output}
        \acro{MU}{multi-user}
        \acro{SER}{symbol error rate}
        \acro{SNR}{signal-to-noise ratio}
        \acro{SVD}{singular value decomposition}
        \acro{OFDM}{orthogonal frequency division multiplexing}
        \acro{EoA}{elevation of arrival}
        \acro{AoA}{azimuth of arrival}
        \acro{EoD}{elevation of departure}
        \acro{AoD}{azimuth of departure}
        \acro{AWGN}{additive white Gaussian noise} 
        \acro{RCS}{radar cross section}
        \acro{ROTR}{Rank-One-Tensor-Receiver}
        \acro{HOSVD}{higher-order singular value decomposition}
        \acro{LOS}{line-of-sight}
        \acro{NLOS}{non-line-of-sight}
        \acro{GLRT}{generalized likelihood ratio test}
        \acro{CRLB}{Cramér–Rao lower bound}
        \acro{Rank-One-Tensor-Receiver}{ROTR}
    \end{acronym}
